PyEquIon: A Python Package For Automatic Speciation Calculations of Aqueous Electrolyte Solutions

In several industrial applications, such as crystallization, pollution control, and flow assurance, an accurate understanding of the aqueous electrolyte solutions is crucial. Electrolyte equilibrium calculation contributes with the design and optimization of processes by providing important information, such as species concentration, solution pH and potential for solid formation. In this work, a pure Python library distributed under BSD-3 license was developed for the calculation of aqueous electrolyte equilibrium. The package takes as inputs the feed components of a given solution, and it automatically identifies its composing ions and the chemical reactions involved to calculate equilibrium conditions. Moreover, there is no established electrolyte activity coefficient model for a broad range of operational conditions. Hence, in this package, built-in activity coefficient models are structured in a modular approach, so that the non-ideality calculation can be performed by a user provided function, which allows further research in the topic. The package can be used by researchers to readily identify the equilibrium reactions and possible solid phases in a user friendly language.

==> img/cases_bromley.tex <==
% This file was created by tikzplotlib v0.8.2.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={(a) $\gamma_{KCl}$},
xlabel={\(\displaystyle m_{KCl} [M]\)},
xmin=-0.24895, xmax=5.24995,
xtick style={color=black},
ymin=0.548386, ymax=0.984734,
ytick style={color=black}
]
\addplot [line width=0.5599999999999999pt, black, mark=square*, mark size=2, mark options={solid}, only marks]
table {%
0.001 0.9649
0.002 0.9515
0.003 0.94162
0.004 0.93356
0.005 0.92664
0.006 0.92054
0.004 0.91504
0.005 0.91003
0.006 0.90541
0.01 0.90111
0.02 0.86885
0.03 0.84672
0.04 0.82959
0.05 0.81553
0.06 0.80358
0.07 0.79317
0.08 0.78394
0.09 0.77566
0.1 0.76815
0.2 0.71696
0.3 0.68653
0.4 0.66526
0.5 0.64919
0.6 0.63646
0.7 0.62607
0.8 0.61741
0.9 0.61008
1 0.60381
1.5 0.58295
2 0.57259
2.5 0.56833
3 0.56822
3.5 0.57116
4 0.57649
4.5 0.58373
5 0.59253
};
\addlegendentry{exp}
\addplot [line width=0.5599999999999999pt, white!40.0!black, dashed, mark=*, mark size=2, mark options={solid}]
table {%
0.001 0.964844970389984
0.002 0.951381238822829
0.003 0.941452194646039
0.004 0.933340872209591
0.005 0.926384039430014
0.006 0.920242439727892
0.004 0.933340872209591
0.005 0.926384039430014
0.006 0.920242439727892
0.01 0.900696995632899
0.02 0.86829452313799
0.03 0.846132892408308
0.04 0.829034509522148
0.05 0.815042257856833
0.06 0.803174886530181
0.07 0.792862023595516
0.08 0.783739795520416
0.09 0.775560617425739
0.1 0.768147827516923
0.2 0.717694195828515
0.3 0.687473657036896
0.4 0.666122771557432
0.5 0.649843433525602
0.6 0.636884694156668
0.7 0.626285548851105
0.8 0.617456574940333
0.9 0.610007526074723
1 0.603665329082092
1.5 0.583024493705231
2 0.573353763579887
2.5 0.569769173518936
3 0.570052476178222
3.5 0.573026687793642
4 0.578002602101077
4.5 0.584547918693295
5 0.592377480422025
};
\addlegendentry{bromley}

\nextgroupplot[
legend cell align={left},
legend style={at={(0.03,0.97)}, anchor=north west, draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={(b) $\gamma_{NaCl}$},
xlabel={\(\displaystyle m_{NaCl} [M]\)},
xmin=-0.08, xmax=6.08,
xtick style={color=black},
ymin=0.6385, ymax=0.9795,
ytick style={color=black}
]
\addplot [line width=0.5599999999999999pt, black, mark=square*, mark size=2, mark options={solid}, only marks]
table {%
0.2 0.77
0.2 0.72
0.2 0.7
0.4 0.68
0.6 0.67
0.8 0.66
1 0.657
1.2 0.654
1.4 0.654
1.6 0.657
1.8 0.661
2 0.667
2.2 0.676
2.4 0.685
2.6 0.687
2.8 0.704
3 0.713
3.2 0.726
3.4 0.739
3.6 0.746
3.8 0.767
4 0.782
4.2 0.799
4.4 0.823
4.6 0.827
4.8 0.854
5 0.873
5.2 0.893
5.4 0.917
5.6 0.93
5.8 0.964
};
\addlegendentry{exp}
\addplot [line width=0.5599999999999999pt, white!40.0!black, dashed, mark=*, mark size=2, mark options={solid}]
table {%
0.2 0.732809400258385
0.2 0.732809400258385
0.2 0.732809400258385
0.4 0.691903504751325
0.6 0.672096385263162
0.8 0.661665995500339
1 0.656753858066601
1.2 0.655552490173851
1.4 0.657054971716529
1.6 0.660640687673529
1.8 0.665901136172863
2 0.672554784183366
2.2 0.680400958354879
2.4 0.689292959103068
2.6 0.699121482120649
2.8 0.709803936525931
3 0.721277312925445
3.2 0.733493278857114
3.4 0.746414720616043
3.6 0.760013252014565
3.8 0.77426738592986
4 0.789161170182003
4.2 0.804683155030771
4.4 0.820825601606103
4.6 0.837583868103182
4.8 0.854955928976247
5 0.872941994910449
5.2 0.891544210051339
5.4 0.910766409100319
5.6 0.930613921263559
5.8 0.951093411212269
};
\addlegendentry{bromley}

\nextgroupplot[
legend cell align={left},
legend style={draw=white!80.0!black},
tick align=outside,
tick pos=left,
title={(c) KCl Solubility [mol/L] in NaCl},
xlabel={\(\displaystyle m_{NaCl} [M]\)},
xmin=0.025452505, xmax=5.065049595,
xtick style={color=black},
ymin=0, ymax=6,
ytick style={color=black}
]
\addplot [line width=0.5599999999999999pt, black, mark=square*, mark size=2, mark options={solid}, only marks]
table {%
4.835977 2.148176
4.581452 2.260164
4.326927 2.376446
4.072402 2.497039
3.817877 2.62195
3.563352 2.751177
3.308827 2.884706
3.054302 3.022514
2.799776 3.164569
2.545251 3.310827
2.290726 3.461239
2.036201 3.615746
1.781676 3.774283
1.527151 3.936778
1.272626 4.103152
1.018101 4.273324
0.7635754 4.447207
0.5090503 4.62471
0.2545251 4.805741
};
\addlegendentry{exp}
\addplot [line width=0.5599999999999999pt, white!40.0!black, dashed, mark=*, mark size=2, mark options={solid}]
table {%
4.835977 2.01232844431851
4.581452 2.11992243827373
4.326927 2.23184803903579
4.072402 2.34813551818096
3.817877 2.46880401177857
3.563352 2.59386145076544
3.308827 2.7233046272915
3.054302 2.85711939369431
2.799776 2.99528153856196
2.545251 3.13775503882192
2.290726 3.28449586046026
2.036201 3.43545043610747
1.781676 3.59055690345624
1.527151 3.7497458646632
1.272626 3.91294118402528
1.018101 4.08006080739294
0.7635754 4.25101800020432
0.5090503 4.42572059326489
0.2545251 4.60407409493887
};
\addlegendentry{bromley}
\end{groupplot}

\end{tikzpicture}

